Beyond the Dashboard: Investigating Distracted Driver Communication Preferences for ADAS

Distracted driving is a major cause of road fatalities. With improvements in driver (in)attention detection, these distracted situations can be caught early to alert drivers and improve road safety and comfort. However, drivers may have differing preferences for the modes of such communication based on the driving scenario and their current distraction state. To this end, we present an (N=147) where videos of simulated driving scenarios were utilized to learn drivers preferences for modes of communication and their evolution with the drivers changing attention. The survey queried participants preferred modes of communication for scenarios such as collisions or stagnation at a green light. that inform the future of communication between drivers and their vehicles. We showcase the different driver preferences based on the nature of the driving scenario and also show that they evolve as the drivers distraction state changes

==> sections/3_hypotheses.tex <==
\section{Hypotheses}
\label{sec:hypothesis}

In this work, we investigate driver preferences for the mode of communication with the ADAS. 
% Our four hypotheses are outlined in Figure \ref{fig:hypothesis_overview}.
% We hypothesize that drivers change their preferred mode of communication based on their distraction state and environmental factors.  
% We also propose that drivers would prefer that their cars autonomously adapt to their (in)attention levels given the driving context.
% Furthermore, we posit that drivers would trust vehicles that implement an adaptive scheme of communication over a standard vehicle.
% Therefore, our four hypotheses are:
Our four hypotheses are:
\begin{enumerate}
    \item[H1] Driver preferences for the mode of communication are based on the hazardous nature of the driving scenario\footnote{We treat this hypothesis as a confirmation hypothesis as the association of modes of communication with their perception by drivers is standardised by multiple transportation authorities~\cite{campbell2018, lerner2015}.}.
    \item[H2] Drivers change their preferred mode of communication as their distraction state changes.
    \item[H3] Drivers prefer that their car autonomously adapt its mode of communication to their changing distraction state. % and preferences.
    \item[H4] Vehicles that implement an adaptive policy for its mode of communication are more trusted by drivers.
\end{enumerate}


% \begin{figure}[t!]
% \centering
%   \subfigure[Hypothesis 1]{\includegraphics[width=0.24\textwidth]{figures/1_1.png}}
%   \subfigure[Hypothesis 2]{\includegraphics[width=0.24\textwidth]{figures/1_2.png}}
%   \subfigure[Hypothesis 3]{\includegraphics[width=0.24\textwidth]{figures/1_3.png}}
%   \subfigure[Hypothesis 4]{\includegraphics[width=0.24\textwidth]{figures/1_4.png}}
%   \caption{The four hypotheses presented: (a) Drivers prefer different modes of communication based on the risk associated in the driving scenario; (b) Drivers change their preferred mode of communication based on their distraction; (c) Drivers prefer that their Advanced Driver Assistance System (ADAS) autonomously adapt its mode of communication to their changing attention; (d) Vehicles that implement an adaptive model of communication would be more trusted by drivers.}
%   % \Description[Pictorial representations of our four hypotheses]{Four images describing the four hypotheses presented in this paper.}
%   \label{fig:hypothesis_overview}
% \end{figure}


% \noindent We treat H1 as a confirmation hypothesis as the association of modes of communication with their perception by drivers is standardised by multiple transportation authorities~\cite{campbell2018, lerner2015}.



